HazyDet: Open-Source Benchmark for Drone-View Object Detection with Depth-Cues in Hazy Scenes

Object detection from aerial platforms under adverse atmospheric conditions, particularly haze, is paramount for robust drone autonomy. Yet, this domain remains largely underexplored, primarily hindered by the absence of specialized benchmarks. To bridge this gap, we present \textit{HazyDet}, the first, large-scale benchmark specifically designed for drone-view object detection in hazy conditions. Comprising 383,000 real-world instances derived from both naturally hazy captures and synthetically hazed scenes augmented from clear images, HazyDet provides a challenging and realistic testbed for advancing detection algorithms. To address the severe visual degradation induced by haze, we propose the Depth-Conditioned Detector (DeCoDet), a novel architecture that integrates a Depth-Conditioned Kernel to dynamically modulate feature representations based on depth cues. The practical efficacy and robustness of DeCoDet are further enhanced by its training with a Progressive Domain Fine-Tuning (PDFT) strategy to navigate synthetic-to-real domain shifts, and a Scale-Invariant Refurbishment Loss (SIRLoss) to ensure resilient learning from potentially noisy depth annotations. Comprehensive empirical validation on HazyDet substantiates the superiority of our unified DeCoDet framework, which achieves state-of-the-art performance, surpassing the closest competitor by a notable +1.5\% mAP on challenging real-world hazy test scenarios. Our dataset and toolkit are available at https://github.com/GrokCV/HazyDet.

==> tables/dataset_compare_count.tex <==

\begin{table}[htbp]
%\vspace{-30pt}
\centering
\captionsetup{font={scriptsize}}
\caption{\textbf{Comprehensive dataset comparison and statistics.} Real and Sim denote real-world and simulated data containing hazy scene, respectively. HazyDet objects are categorized by area-to-image ratio: small (<0.1\%), medium (0.1\%--1\%), and large (>1\%).}
\label{tab:dataset_compare_count}
%\vspace{6pt}

\begin{subtable}[t]{0.526\linewidth}
\resizebox{1\linewidth}{!}{
\begin{tabular}{lccccccc}  
  \toprule  
  Dataset                                   & Usage    & Real     & Sim      & Scenes    & Images & Annotations  & Year \\
  \midrule  
  VEDAI \citep{JVCIR2016VEDAI}              & Det      & $\times$      & $\times$      & Drone     & 1,200  & 3,700      & 2016 \\
  CAPRK \citep{ICCV2017CAPRK}               & Det      & $\times$      & $\times$      & Drone     & 1,448  & 89,777     & 2017 \\
  VisDrone \citep{TPAMI2022VisDrone}        & Det      & $\times$      & $\times$      & Drone     & 10,209 & 343,173    & 2022 \\
  D-HAZE \citep{ICIP2016Dhzae}              & Res   & $\times$      & \checkmark    & Normal    & 1,449  & NO         & 2016 \\
  % O-HAZE\citep{CVPRW2018OHaze}              & $\times$      & \checkmark    & Normal    & 45     & NO         & 2018 \\
  Dense-HAZE\citep{ICIP2019DenseHazes}      & Res   & $\times$      & \checkmark    & Normal    & 95     & NO         & 2019 \\
  RESIDE \citep{TIP2019RESIDE}              & Res   & $\times$      & \checkmark    & Normal    & 13,990 & NO         & 2019 \\
  4KDehaze \citep{CVPR2021_4KDehaze}        & Res   & $\times$      & \checkmark    & Normal    & 8,200  & NO         & 2021 \\
  RS-Haze \citep{TIP2023RSHaze}             & Res   & $\times$      & \checkmark    & Satellite & 50,000 & NO         & 2023 \\
  RW-Haze \citep{TMM2023RW-HAZE}            & Res   & \checkmark    & $\times$      & Normal    & 210    & NO         & 2023 \\
  RTTS \citep{TIP2019RESIDE}                & Det      & \checkmark    & $\times$      & Normal    & 4,322  & 41,203     & 2019 \\
  A2I2 \citep{TIP2023A2I2}                  & Det      & \checkmark    & $\times$      & Drone     & 359    & 3,898      & 2023 \\
  {\cellcolor[rgb]{0.929,0.929,0.929}}\textbf{HazyDet} & {\cellcolor[rgb]{0.929,0.929,0.929}}det & {\cellcolor[rgb]{0.929,0.929,0.929}}\checkmark & {\cellcolor[rgb]{0.929,0.929,0.929}}\checkmark & {\cellcolor[rgb]{0.929,0.929,0.929}}Drone & {\cellcolor[rgb]{0.929,0.929,0.929}}11,600 & {\cellcolor[rgb]{0.929,0.929,0.929}}383,689 & {\cellcolor[rgb]{0.929,0.929,0.929}}2025 \\
  \bottomrule  
\end{tabular}
}
\caption{Comparison of related datasets.}
\end{subtable}
\hfill
\begin{subtable}[t]{0.46\linewidth}
\resizebox{1\linewidth}{!}{  
\begin{tabular}{lccclccc}  
    \toprule  
    Split &  
    Images&  
    Objects &  
   Class& Small & Medium & Large \\
    \midrule  
    \multirow{3}{*}{Train} & \multirow{3}{*}{8,000} & \multirow{3}{*}{264,511}  
      & Car   & 159,491 & 77,527 & 5,177 \\
    & & & Truck & 4,197   & 6,262  & 1,167 \\
    & & & Bus   & 1,990   & 7,879  & 861   \\
    \midrule  
    \multirow{3}{*}{Val}   & \multirow{3}{*}{1,000} & \multirow{3}{*}{34,560}  
      & Car   & 21,051  & 9,881  & 630   \\
    & & & Truck & 552     & 853    & 103   \\
    & & & Bus   & 243     & 1,122  & 125   \\
    \midrule  
    \multirow{3}{*}{Test}  & \multirow{3}{*}{2,000} & \multirow{3}{*}{65,322}  
      & Car   & 38,910  & 19,860 & 1,256 \\
    & & & Truck & 881     & 1,409  & 263   \\
    & & & Bus   & 473     & 1,991  & 279   \\
    \midrule  
    \multirow{3}{*}{Real-world} & \multirow{3}{*}{600} & \multirow{3}{*}{19,296}  
      & Car   & 8,167   & 8,993  & 1,060 \\
    & & & Truck & 112     & 290    & 87    \\
    & & & Bus   & 69      & 363    & 155   \\
    \bottomrule  
\end{tabular}
}
\caption{Detailed composition analysis of the HazyDet dataset.}
\end{subtable}
\vspace{-4em}
\end{table}



